Vid3D: Synthesis of Dynamic 3D Scenes using 2D Video Diffusion

A recent frontier in computer vision has been the task of 3D video generation, which consists of generating a time-varying 3D representation of a scene. To generate dynamic 3D scenes, current methods explicitly model 3D temporal dynamics by jointly optimizing for consistency across both time and views of the scene. In this paper, we instead investigate whether it is necessary to explicitly enforce multiview consistency over time, as current approaches do, or if it is sufficient for a model to generate 3D representations of each timestep independently. We hence propose a model, Vid3D, that leverages 2D video diffusion to generate 3D videos by first generating a 2D "seed" of the video's temporal dynamics and then independently generating a 3D representation for each timestep in the seed video. We evaluate Vid3D against two state-of-the-art 3D video generation methods and find that Vid3D is achieves comparable results despite not explicitly modeling 3D temporal dynamics. We further ablate how the quality of Vid3D depends on the number of views generated per frame. While we observe some degradation with fewer views, performance degradation remains minor. Our results thus suggest that 3D temporal knowledge may not be necessary to generate high-quality dynamic 3D scenes, potentially enabling simpler generative algorithms for this task.

==> sec/proposal.tex <==
\label{sec:proposal}
\section{Motivation}
A central theme from the field of computer vision has been the advancement of the modalities and tasks modeled: from classification to generation, static scenes to videos, and from 2D representations to 3D representations~\citep{brooks2024sora, kerbl2023splatting, mildenhall2020nerf}.
A natural next step in developing vision models that more accurately represent the true structure of world is thus unifying generation, dynamic scenes, and 3D representations by developing generative 3D models.
However, there is no general 3D video dataset on which to train such models.
In this work, we plan to take an important first step towards general 3D video models by constructing the first general dataset 3D video dataset.
We believe this work to be important as dynamic 3D scenes can be leveraged in many downstream applications such as embodied robotics, movie generation, and video game development.

\section{Related Work}

Constructing large 3D shape datasets has been a long-standing goal in computer vision~\citep{shapenet2015}. 
To automate and thus scale the building of static 3D scene datasets, researchers have recently leveraged advances in generative 2D video models to generate static 3D scenes by querying a video model for multiple poses of the said scene~\citep{chen2024v3d, han2024vfusion3d}.
However, these existing methods only generate static 3D data, meaning that there is no temporal component.
Some existing highly domain-specific 3D video datasets (i.e. human bodies, human faces, etc.) have been manually curated using a large number of sensors~\citep{chatzitofis2020human4d, reimat2021cwipc, yoon2021humbi, pages2021volograms}.
The use of these 3D video datasets is limited due to their domain-specific nature.
Additionally, it is hard to scale their hardware-intensive video capture technology to produce larger datasets.
All the datasets listed above, as well as the code from \citet{chen2024v3d}, are publicly available.


\section{Proposed Approach}

We propose to generate 3D videos in a two-step process: (1) sample 2D videos and (2) convert each 2D frame to a 3D representation.
This process will allow us to generate diverse 3D videos due to the generality of 2D video models.

To generate short object-centric 2D videos we plan to use the open source Stable Video Diffusion model~\citep{blattmann2023stable}.
For each frame in the resulting video, we will apply the 2D to 3D modeling process proposed by~\citet{chen2024v3d} as it is the state of the art for general 2D to 3D modeling.

The process detailed above will yield a 3D representation for every frame, but the resulting data may not have sufficient fidelity or frame-by-frame consistency to be a high-quality dataset.
To improve the quality of the data, we will first use standard filtering techniques, such as 3D antialiasing ~\citep{liang2024analyticsplatting}, before training a graph neural network to smooth the point clouds between frames. 
We believe that this novel graph neural network architecture will be successful for smoothing, as graph neural networks can naturally represent spatial dependence between point clouds ~\citep{10.1115/1.4064673}.
We will also manually label the quality of a subset of the 3D videos from which we can train a simple quality classifier to filter the dataset by.

We plan to train/run all models on 128 A100-80GB GPUs that we have access to through Databricks Mosaic AI.
\section{Evaluation}

All data created will be evaluated using human preferences, as ours is the first work on general 3D videos, so there is no standard benchmark or metric.
Renderings of dynamic 3D objects will be provided to a subset of humans to be graded on several axes, such as coherency, realism, etc., taking inspiration from other holistic benchmarks ~\citep{lee2023holistic}.
Human evaluation is intrinsically limited by the bias of human judges, which is an unavoidable factor given the absence of objective benchmarks.
We will also include renderings of the 3D videos in our paper.

\section{Contribution}

If this project is successful, we anticipate the 3D video dataset to enable further research into the synthetic generation of data that can better model real-world scenes through time.
This would be the first general 3D video dataset and as such will enable many downstream applications and could lead to the production of more rich and contextual world models, such as in robotics, which depend on large quantities of high-fidelity real-world data.
